PAC Learning Linear Thresholds from Label Proportions

Learning from label proportions (LLP) is a generalization of supervised learning in which the training data is available as sets or bags of feature-vectors (instances) along with the average instance-label of each bag. The goal is to train a good instance classifier. While most previous works on LLP have focused on training models on such training data, computational learnability of LLP was only recently explored by [Saket'21, Saket'22] who showed worst case intractability of properly learning linear threshold functions (LTFs) from label proportions. However, their work did not rule out efficient algorithms for this problem on natural distributions. In this work we show that it is indeed possible to efficiently learn LTFs using LTFs when given access to random bags of some label proportion in which feature-vectors are, conditioned on their labels, independently sampled from a Gaussian distribution $N(\mathbf{\mu}, \mathbf{\Sigma})$. Our work shows that a certain matrix -- formed using covariances of the differences of feature-vectors sampled from the bags with and without replacement -- necessarily has its principal component, after a transformation, in the direction of the normal vector of the LTF. Our algorithm estimates the means and covariance matrices using subgaussian concentration bounds which we show can be applied to efficiently sample bags for approximating the normal direction. Using this in conjunction with novel generalization error bounds in the bag setting, we show that a low error hypothesis LTF can be identified. For some special cases of the $N(\mathbf{0}, \mathbf{I})$ distribution we provide a simpler mean estimation based algorithm. We include an experimental evaluation of our learning algorithms along with a comparison with those of [Saket'21, Saket'22] and random LTFs, demonstrating the effectiveness of our techniques.

==> misclassification_bound.tex <==
\section{Bounding Classification Error} \label{sec:misclassification_bound}

\begin{theorem}
For any $\eps' \in (0,1]$ there exists $\eps \in (0, 1]$ s.t. if $\|\br - \hat{\br}\|_2 \leq \eps$ for any unit vectors $\br, \hat{\br}$, then $\Pr\left[\pos\left(\br^T\bX\right)\neq \pos\left(\hat{\br}^T\bX\right)\right] \leq \eps'$.
\end{theorem}


==> table_non_std_gaussian_experiments.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{d}} & \multicolumn{1}{c|}{\textbf{q, k}} & \multicolumn{1}{c|}{\textbf{m}} & \multicolumn{1}{c|}{\textbf{A2}} & \multicolumn{1}{c|}{\textbf{R}} \\ \hline
             &               & 100                             & 91.25\errbar{0.19}                       & 74.75\errbar{0.46}                      \\ \cline{3-5} 
                                 &  2, 1                                  & 500                             & 96.26\errbar{0.02}                       & 76.86\errbar{0.23}                      \\ \cline{3-5} 
                                 &                                    & 2000                            & 98.18\errbar{0.01}                       & 78.32\errbar{0.23}                      \\ \cline{2-5} 
                                 &               & 100                             & 90.44\errbar{0.12}                       & 70.64\errbar{1.09}                      \\ \cline{3-5} 
                                 & 3, 1                                   & 500                             & 96.04\errbar{0.04}                       & 73.32\errbar{1.1}                       \\ \cline{3-5} 
                                 &                                    & 2000                            & 97.92\errbar{0.01}                       & 75.14\errbar{0.47}                      \\ \cline{2-5} 
                                 &              & 100                             & 89.36\errbar{0.23}                       & 66.08\errbar{0.98}                      \\ \cline{3-5} 
                                 & 10, 5                                   & 500                             & 95.48\errbar{0.02}                       & 69.46\errbar{0.99}                      \\ \cline{3-5} 
10                                 &                                    & 2000                            & 97.86\errbar{0.01}                       & 70.41\errbar{0.86}                      \\ \cline{2-5} 
                                 &              & 100                             & 85.97\errbar{0.3}                        & 63.39\errbar{0.84}                      \\ \cline{3-5} 
                                 & 10, 8                                   & 500                             & 94.02\errbar{0.1}                        & 69.71\errbar{0.58}                      \\ \cline{3-5} 
                                 &                                    & 2000                            & 97.4\errbar{0.01}                        & 69.86\errbar{0.8}                       \\ \cline{2-5} 
                                 &             & 100                             & 87.92\errbar{0.28}                       & 60.65\errbar{0.6}                       \\ \cline{3-5} 
                                 & 50, 25                                   & 500                             & 95.5\errbar{0.03}                        & 61.73\errbar{0.8}                       \\ \cline{3-5} 
                                 &                                    & 2000                            & 97.57\errbar{0.02}                       & 70.48\errbar{0.69}                      \\ \cline{2-5} 
                                 &             & 100                             & 89.12\errbar{0.18}                       & 59.08\errbar{0.52}                      \\ \cline{3-5} 
                                 & 50, 35                                   & 500                             & 95.2\errbar{0.03}                        & 60.67\errbar{0.62}                      \\ \cline{3-5} 
                                 &                                    & 2000                            & 97.6\errbar{0.01}                        & 62.86\errbar{0.75}                      \\ \hline
             &               & 100                             & 69.08\errbar{0.46}                       & 55.44\errbar{0.21}                      \\ \cline{3-5} 
                                 & 2, 1                                   & 500                             & 89.46\errbar{0.12}                       & 57.35\errbar{0.32}                      \\ \cline{3-5} 
                                 &                                    & 2000                            & 94.99\errbar{0.03}                       & 58.68\errbar{0.15}                      \\ \cline{2-5} 
                                 &               & 100                             & 66.42\errbar{1.59}                       & 57.24\errbar{0.46}                      \\ \cline{3-5} 
                                 & 3, 1                                   & 500                             & 89.96\errbar{0.23}                       & 57.22\errbar{0.28}                      \\ \cline{3-5} 
                                 &                                    & 2000                            & 95.6\errbar{0.05}                        & 59.8\errbar{0.84}                       \\ \cline{2-5} 
                                 &              & 100                             & 65.76\errbar{1.07}                       & 54.71\errbar{0.13}                      \\ \cline{3-5} 
                                 & 10, 5                                   & 500                             & 90.2\errbar{0.14}                        & 56.57\errbar{0.25}                      \\ \cline{3-5} 
50                                 &                                    & 2000                            & 95.27\errbar{0.04}                       & 57.43\errbar{0.13}                      \\ \cline{2-5} 
                                 &              & 100                             & 62.48\errbar{0.7}                        & 62.27\errbar{0.82}                      \\ \cline{3-5} 
                                 & 10, 8                                   & 500                             & 88.04\errbar{0.29}                       & 61.4\errbar{0.49}                       \\ \cline{3-5} 
                                 &                                    & 2000                            & 94.44\errbar{0.06}                       & 61.82\errbar{0.54}                      \\ \cline{2-5} 
                                 &             & 100                             & 65.07\errbar{0.81}                       & 54.78\errbar{0.14}                      \\ \cline{3-5} 
                                 & 50, 25                                   & 500                             & 87.72\errbar{0.28}                       & 55.22\errbar{0.22}                      \\ \cline{3-5} 
                                 &                                    & 2000                            & 94.97\errbar{0.02}                       & 53.98\errbar{0.08}                      \\ \cline{2-5} 
                                 &             & 100                             & 66.12\errbar{0.67}                       & 56.97\errbar{0.28}                      \\ \cline{3-5} 
                                 & 50, 35                                   & 500                             & 87.86\errbar{0.17}                       & 59.57\errbar{0.3}                       \\ \cline{3-5} 
                                 &                                    & 2000                            & 94.33\errbar{0.03}                       & 56.97\errbar{0.32}                      \\ \hline
\end{tabular}
\caption{Our algorithm A2 vs. rand. LTF (R) on $N(\bm{\mu}, \bm{\Sigma})$ feature vectors}
\label{tab:non_std_gaussian_experiments}
\end{table}

==> table_sdp_experiments.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{q, k}} & \multicolumn{1}{c|}{\textbf{d}} & \multicolumn{1}{c|}{\textbf{m}} & \multicolumn{1}{c|}{\textbf{S}} \\ \hline
               &              & 50                              & 77.44\errbar{6.58}                      \\ \cline{3-4} 
                                    & 10                                & 100                             & 84.31\errbar{5.32}                      \\ \cline{3-4} 
2, 1                                    &                                 & 200                             & 90.1\errbar{4.15}                       \\ \cline{2-4} 
                                    &              & 50                              & 59.58\errbar{3.89}                      \\ \cline{3-4} 
                                    & 50                                & 100                             & 59.95\errbar{3.17}                      \\ \cline{3-4} 
                                    &                                 & 200                             & 61.12\errbar{4.29}                      \\ \hline
               &              & 50                              & 72.08\errbar{6.59}                      \\ \cline{3-4} 
                                    & 10                                & 100                             & 71.58\errbar{8.22}                      \\ \cline{3-4} 
3, 1                                    &                                 & 200                             & 70.8\errbar{7.52}                       \\ \cline{2-4} 
                                    &              & 50                              & 63.9\errbar{7.46}                       \\ \cline{3-4} 
                                    & 50                                & 100                             & 62.69\errbar{6.75}                      \\ \cline{3-4} 
                                    &                                 & 200                             & 62.39\errbar{7.67}                      \\ \hline
\end{tabular}
\caption{SDP algorithm S on $N(\bm{\mu}, \bm{\Sigma})$ feature vectors}
\label{tab:sdp_experiments}
\end{table}

==> table_std_gaussian_experiments.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{d}} & \multicolumn{1}{c|}{\textbf{q, k}} & \multicolumn{1}{c|}{\textbf{m}} & \multicolumn{1}{c|}{\textbf{A1}} & \multicolumn{1}{c|}{\textbf{A2}} & \multicolumn{1}{c|}{\textbf{R}} \\ \hline
              &               & 100                             & 82.37\errbar{0.13}                       & 90.2\errbar{0.07}                        & 73.46\errbar{0.68}                      \\ \cline{3-6} 
                                 &  3, 1                                  & 500                             & 91.2\errbar{0.03}                        & 96.34\errbar{0.01}                       & 73.26\errbar{0.34}                      \\ \cline{3-6} 
                                 &                                    & 2000                            & 95.52\errbar{0.01}                       & 98.17\errbar{0.0}                        & 76.0\errbar{0.15}                       \\ \cline{2-6} 
                                 &              & 100                             & 94.28\errbar{0.02}                       & 87.48\errbar{0.59}                       & 74.73\errbar{0.2}                       \\ \cline{3-6} 
10                                 & 10, 8                                   & 500                             & 96.96\errbar{0.01}                       & 95.29\errbar{0.01}                       & 74.76\errbar{0.13}                      \\ \cline{3-6} 
                                 &                                    & 2000                            & 98.58\errbar{0.0}                        & 97.68\errbar{0.0}                        & 75.46\errbar{0.12}                      \\ \cline{2-6} 
                                 &             & 100                             & 95.79\errbar{0.01}                       & 89.99\errbar{0.07}                       & 73.34\errbar{0.5}                       \\ \cline{3-6} 
                                 & 50, 35                                   & 500                             & 98.26\errbar{0.0}                        & 95.63\errbar{0.03}                       & 72.83\errbar{0.22}                      \\ \cline{3-6} 
                                 &                                    & 2000                            & 99.06\errbar{0.0}                        & 97.95\errbar{0.01}                       & 74.18\errbar{0.22}                      \\ \hline
              &               & 100                             & 67.75\errbar{0.11}                       & 61.21\errbar{0.63}                       & 55.34\errbar{0.11}                      \\ \cline{3-6} 
                                 & 3, 1                                   & 500                             & 80.78\errbar{0.05}                       & 89.45\errbar{0.02}                       & 56.72\errbar{0.17}                      \\ \cline{3-6} 
                                 &                                    & 2000                            & 89.26\errbar{0.02}                       & 95.15\errbar{0.01}                       & 59.86\errbar{0.09}                      \\ \cline{2-6} 
                                 &              & 100                             & 85.7\errbar{0.02}                        & 60.4\errbar{0.53}                        & 56.26\errbar{0.12}                      \\ \cline{3-6} 
50                                 & 10, 8                                   & 500                             & 94.09\errbar{0.01}                       & 86.84\errbar{0.04}                       & 60.37\errbar{0.11}                      \\ \cline{3-6} 
                                 &                                    & 2000                            & 96.73\errbar{0.0}                        & 94.36\errbar{0.01}                       & 61.58\errbar{0.07}                      \\ \cline{2-6} 
                                 &             & 100                             & 90.21\errbar{0.02}                       & 62.8\errbar{0.52}                        & 55.84\errbar{0.1}                       \\ \cline{3-6} 
                                 & 50, 35                                   & 500                             & 95.68\errbar{0.01}                       & 89.09\errbar{0.03}                       & 59.69\errbar{0.15}                      \\ \cline{3-6} 
                                 &                                    & 2000                            & 97.82\errbar{0.0}                        & 94.94\errbar{0.01}                       & 61.04\errbar{0.14}                      \\ \hline
\end{tabular}
\caption{Our algorithms A2 and A3 vs . rand. LTF (R) on $N(\bm{0}, \bm{I})$ feature vectors}
\label{tab:std_gaussian_experiments}
\end{table}
